Unsupervised Opinion Summarization Using Approximate Geodesics

Opinion summarization is the task of creating summaries capturing popular opinions from user reviews. In this paper, we introduce Geodesic Summarizer (GeoSumm), a novel system to perform unsupervised extractive opinion summarization. GeoSumm involves an encoder-decoder based representation learning model, that generates representations of text as a distribution over latent semantic units. GeoSumm generates these representations by performing dictionary learning over pre-trained text representations at multiple decoder layers. We then use these representations to quantify the relevance of review sentences using a novel approximate geodesic distance based scoring mechanism. We use the relevance scores to identify popular opinions in order to compose general and aspect-specific summaries. Our proposed model, GeoSumm, achieves state-of-the-art performance on three opinion summarization datasets. We perform additional experiments to analyze the functioning of our model and showcase the generalization ability of {\X} across different domains.

==> tables/human_eval_aspect_space.tex <==
\resizebox{0.37\textwidth}{!}{
	\begin{tabular}{ l c  c c} 
		\toprule[1pt]
		 Aspect  & {Exclusive} & {Partial} & {None} \Tstrut\\ 			
		\midrule[1pt]
        {AceSum}  & 50.9 & 42.6 & 6.5\\
        {\X} & 22.5 & 66.4 & 11.1\\
		{SemAE} &  ~~\textbf{70.7}* & ~~\textbf{25.9}* & ~~\textbf{3.4}*\\
		\bottomrule[0.5pt]
	\end{tabular}
}


==> tables/human_eval_general_oposum.tex <==
\resizebox{0.39\textwidth}{!}{
	\begin{tabular}{ l c  c c} 
		\toprule[1pt]
		 General  & {Inform.} & {Coherence} & {Redund.} \Tstrut\\ 			
		\midrule[1pt]
		{SemAE} & 31.7 & -13.3 & -16.1\Tstrut\\
        {AceSum}  & -53.9 & \textbf{7.2} & \textbf{21.7}\\
		{\X} &  {5.0} & 6.1 & -5.6\Bstrut\\
		\bottomrule[0.5pt]
	\end{tabular}
}
